On Fairness Concerns in the Blockchain Ecosystem

Blockchains revolutionized centralized sectors like banking and finance by promoting decentralization and transparency. In a blockchain, information is transmitted through transactions issued by participants or applications. Miners crucially select, order, and validate pending transactions for block inclusion, prioritizing those with higher incentives or fees. The order in which transactions are included can impact the blockchain final state. Moreover, applications running on top of a blockchain often rely on governance protocols to decentralize the decision-making power to make changes to their core functionality. These changes can affect how participants interact with these applications. Since one token equals one vote, participants holding multiple tokens have a higher voting power to support or reject the proposed changes. The extent to which this voting power is distributed is questionable and if highly concentrated among a few holders can lead to governance attacks. In this thesis, we audit the Bitcoin and Ethereum blockchains to investigate the norms followed by miners in determining the transaction prioritization. We also audit decentralized governance protocols such as Compound to evaluate whether the voting power is fairly distributed among the participants. Our findings have significant implications for future developments of blockchains and decentralized applications.

==> chapters/5_governance/3b_voting_modalities.tex <==
% !TEX root = ../../thesis.tex
%


\section{Voting modalities}\label{subsec:background-voting-modalities}


Proposals to change a governance protocol takes birth in the protocol's community forum.
%
Community members suggest and discuss potential changes to the protocol in the forum and may even conduct an informal poll to gauge the community's support for a proposal.
%
The proposer then either amends the proposal to incorporate the community's feedback and submit it for a formal vote, or simply abandon it.
%
The formal voting on the proposal has two modes: \stress{on-chain} and \stress{off-chain} voting.

\paraib{On-chain voting}
%
In this voting system, participants make all governance decisions via smart contracts on a blockchain.
%
Under this system, participants cast a vote by issuing a transaction (and paying a fee for committing it) to the blockchain.
%
The system allows only participants with at least a threshold amount of (governance) tokens to create a proposal, albeit any token holding participant can vote on that proposal.
%
It executes the proposal on the blockchain only if it receives a significant number of votes in favor and reaches a \stress{quorum}.
%
This voting system thus facilitates making transparent and tamper-proof changes to the protocol.
%
Decentralized governance protocols such as AAVE~\cite{Governance@AAVE}, Compound~\cite{Governance@Compound}, and Uniswap~\cite{Governance@Uniswap} use on-chain voting.

\paraib{Off-Chain Voting}
%
This system conducts voting on an off-chain third-party platform and, as a consequence, also establishes the rules for voting, aggregating votes, and determining the results off-chain.
%
Protocols such as Balancer~\cite{Governance@Balancer} and Convex Finance~\cite{Governance@ConvexFinance}, for instance, use Snapshot~\cite{Snapshot} for off-chain voting.
%
Snapshot stores the voting data on a P2P network called InterPlanetary File System (IPFS)~\cite{IPFS}.
%
The voting process does not require voters to pay any fees and (unlike on-chain voting) promotes participation across all participants, regardless of their level of participation or investment in the protocol.
%
After the voting, this system uses a \stress{multi-signature} contract to enact the off-chain voting outcome on the blockchain.
%
Typically, an \stress{n-of-m multisig} contract requires the transaction to be signed by at least \stress{n} out of the \stress{m} ``admins'' to be executed on-chain.
%
The system trusts the multisig ``admins'', who are well-known in the community, to implement the voting outcome on the blockchain truthfully.
%
The admins can also, however, refuse the protocol.
%
In Convex Finance, for instance, the admins can choose not to execute a proposal if they deem it harmful, even if it had received the majority of votes and reached a quorum~\cite{Docs@ConvexFinance}.
%
On-chain voting systems, in contrast, prevent such manipulation of voting outcomes by one or more individuals (after the voting process), since all governance decisions (e.g., voting and execution) happen on the chain.


\paraib{Token delegations}
%
Some governance protocols (e.g., Compound, Uniswap, and AAVE) require a user to own a certain amount of governance tokens for casting a vote.
%
Users must delegate their tokens either to themselves or, if they do not wish to vote, delegate them to others.
%
The ability to delegate voting power to others facilitates a form of liquid democracy; the token holder who delegates or sells their tokens to another loses their voting power.
%
Delegations allow anyone to buy (or sell) tokens and gain (or lose) voting power instantly.
%
Justin Sun, the founder of (stablecoin) TrueUSD~\cite{TrueUSD}, for instance, allegedly borrowed COMP tokens to create and vote for Compound proposal \#84~\cite{Proposal-84@Compound}, resulting in a \stress{governance attack}~\cite{Thurman@Coindesk}; this proposal was, however, defeated.


\paraib{Token ``locking''}
%
Protocols such as Balancer and Curve~\cite{Governance@Curve} mandate that a user ``lock'' their tokens into a smart contract for a specified period of time to gain their right to vote.
%
The user cannot withdraw the locked tokens until the lock-up period expires.
%
The voting power of a user in this system is proportional to the amount of tokens locked as well as the lock-up period.
%
In Balancer, for instance, a user receives \num{1} unit of voting power if they lock \num{1} token into the contract for \num{1} year, and only half that voting power if they lock it instead for \num{6} months.

\paraib{Continuous voting}
%
A few protocols (e.g., MakerDAO~\cite{Governance@MakerDAO}) allow voters to change their votes at any time during the voting period.
%
Users propose a protocol change by developing a new implementation via a smart contract.
%
The new implementation is accepted if it receives more votes than the current one, i.e., the winning implementation must always receive the majority of the votes (or tokens).
%
MakerDAO requires a user to deposit their (MKR) tokens into the (Maker) Governance contract for casting a vote.
%
The more tokens they deposit, the more voting power they obtain, and they vote for their desired implementation by specifying it as a protocol parameter in the smart contract.
%
Since the voting process is continuous, if a user withdraws their MKR tokens from the governance contract, their vote will no longer count towards the implementations for which they previously voted.

We refer the reader to \S\ref{sec:types-of-governance} (particularly Table~\ref{table:protocol-types}) for a characterization of the voting methods, delegation approaches, and proposal executions in various other governance protocols.
%
Understanding how voting is conducted (i.e., whether it is on-chain or off-chain) and proposals are executed is fundamental for analyzing how voters, proposers, and others interact with these governance protocols.



==> frontmatter/12_abbreviations.tex <==
\phantomsection
\addcontentsline{toc}{chapter}{LIST OF ABBREVIATIONS}

\begin{center}
{\Large \textbf{LIST OF ABBREVIATIONS}}
\end{center}

\newcommand{\Ab}[2]{\noindent  #1 \> #2 \\}
\newcommand{\Abi}[2]{\noindent #1 \hspace{1.5cm} \= #2 \\}

\begin{tabbing}

\end{tabbing}

\clearpage


==> frontmatter/preface.tex <==
\begin{center}
{\Large \textbf{PREFACE}}
\end{center}


\tbw


\clearpage

